Beyond socket options: making the Linux TCP stack truly extensible

The Transmission Control Protocol (TCP) is one of the most important protocols in today's Internet. Its specification and implementations have been refined for almost forty years. The Linux TCP stack is one of the most widely used TCP stacks given its utilisation on servers and Android smartphones and tablets. However, TCP and its implementations evolve very slowly. In this paper, we demonstrate how to leverage the eBPF virtual machine that is part of the recent versions of the Linux kernel to make the TCP stack easier to extend. We demonstrate a variety of use cases where the eBPF code is injected inside a running kernel to update or tune the TCP implementation. We first implement the TCP User Timeout Option. Then we propose a new option that enables a client to request a server to use a specific congestion control scheme. Our third extension is a TCP option that sets the initial congestion window. We then demonstrate how eBPF code can be used to tune the acknowledgment strategy.

==> mptcp.tex <==
\section {Extending Multipath TCP}
\label{s:mptcp}

Above sections have illustrated how we extend the TCP-BPF to allow user daemons to support new TCP options dynamically. This section will show that this framework can be adapted easily to support new MPTCP options. But before that, we need the ability to track and control each subflow, not only the aggregated MPTCP connection.

\subsection{Tracking MPTCP subflows}

Multipath TCP logically includes two sublayers: one or several subflows which appear to the network infrastructure as separated TCP connections, and meta connection which appears to the application as a regular TCP connection.

To track the subflows, we can just use the TCP-BPF callbacks already available in the kernel. However, the called BPF program does not have any MPTCP-specific information to make any wise decision. For this reason, we need to add MPTCP-specific hooks at the right place.

On the Linux client side, when a new subflow is created, the stack initializes its meta-level information and add the subflow socket into the MPTCP connection by \texttt{mptcp\_add\_sock()}. By a hook in this function we can start tracking the subflow with the \texttt{sock} structure.

On the client side, a master subflow is established when \texttt{MP\_CAPABLE SYN-ACK} arrived, and a joined subflow is established when \texttt{MP\_JOIN SYN-ACK} arrived. Interestingly in both cases, \texttt{mptcp\_rcv\_synsent\_state\_process()} is called to finish the subflow establishment. So, we only need to add a single hook to track the establishment of both master subflow and joined subflows. We also passed the subflow ID to the BPF program, so that the BPF program knows it is the master subflow or a joined subflow.

\subsection{Supporting new MPTCP options}

\subsubsection{At sender: Inserting a new option}

To enable or disable option-writing action at any phase of a subflow, the same flag array \texttt{bpf\_sock\_ops\_cb\_flags} is used. If we pass the TCP subflow sock in the context, the program will control the option-writing action per subflow basis.

To actually insert new options, we may reuse our facilities for TCP (as mentioned in \ref{sss:insert-tcp-opt}). However, to explicitly insert MPTCP options only, we used an MPTCP-specific hook in \texttt{mptcp\_options\_write()} instead.

\subsubsection{At receiver: Parsing a new MPTCP option}
To parse new MPTCP option, we cannot reuse our TCP hook (mentioned in \ref{sss:parse-tcp-opt}) which only processes regular TCP options. Instead, MPTCP options are processed in \texttt{mptcp\_parse\_options()}. Therefore, at the end of this function, when encounter an unknown MPTCP option, we pass the option subtype, the length and the option data to the BPF program.

\section{MPTCP Use Cases}
\label{s:mptcp-usecase}

\subsection{Client Requests Server to Cap Bandwidth on a Subflow}

\textit{Motivation:} A common scenario for the mobile users subscribed to metered cellular packages is when they want to limit the monetary cost of using  cellular networks. For this, the client may requests server to cap bandwidth on the cellular network subflow.

At first, on the client side, the BPF program needs to select which subflow to send the MPTCP option to cap bandwidth. For that, the kernel stack needs to pass the type of interface (net\_device.type) to the BPF program. We considered different ways to achieve this:

We can retrieve the device type from outgoing packets (skb.skb\_iif), then pass it to the BPF program. This is simple but expensive since the BPF program will be called on the fast path for every outgoing segment.

We can retrieve from the sock struct, when a new sub sock is added by mptcp\_add\_sock(). However, this will not work, since at this point the subflow join SYN has not even been sent, it is not a full sock which is required by the TCP-BPF framework.


Our solution is to get device type from SYN-ACK skb. We added a hook when receiving an MPTCP SYN-ACK (in mptcp\_rcv\_synsent\_state\_process()). This is triggered when we receive either MP\_CAPABLE or MP\_JOIN. We also passed the subflow ID to the BPF program, so that the BPF program knows it is the master subflow or a joined subflow.


If the BPF program sees that this subflow is on the cellular interface, it will activate the option-writing flag on this subflow.
After that, when the MPTCP stack sends a packet on the marked subflow, the BPF program will write an MPTCP option on this outgoing packet. This new MPTCP option signals the server to cap the bandwidth on this subflow. 

When the server receives a bw\_cap option on a subflow, the BPF program parses this value and also gets smoothed RTT and MSS values from tcp\_sock, base on which, it calculates the right cwnd\_clamp needed to apply on this subflow.
Since the RTT may change over the time, we need to monitor RTT and adjust the cwnd\_clamp. A simple solution is letting the client send the option on every outgoing packet that triggers the server to update cwnd\_clamp continually. To reduce the overhead, the client can send option periodically e.g.: every 10 segments or every 10 seconds.

\begin{figure}
	\centering
	\includegraphics[width=0.7\linewidth]{figures/cap-bw}
	\caption{Raw throughput on the second path, before and after capping 100 KBps.}
	\label{fig:cap-bw}
\end{figure}


\subsection{Delay threshold option for thin streams}

\textit{Motivation:} For thin streams, e.g. those created
by the voice recognition application, we want to maintain the
low latency. We may use redundant scheduler on both sides,
but on mobile devices we do not want consume cellular traffic
as long as the delay on WiFi path is still good enough.

The basic idea is, the client tells the server the delay value that the server should keep as upper threshold. When the current RTT surpasses this theshold, the server would start sending data over the secondary subflow.


At the beginning, the client needs to signal the server to set additional subflows as backup join SYNs will be marked with backup flag = 1. Then, the receiver will set the joined subflows into the backup mode.

The new MPTCP option includes an RTT value in milliseconds.
The option is sent on the master subflow only, and only after joined subflow has been established.

On server, we added a field in mptcp\_cb to stores the RTT threshold value per MPTCP connection. When server receives the option which containing the RTT threshold value, the bpf program is called to set remember this RTT threshold in mptcp\_cb.

When the server receives a new ACK and calculates the new smoothed RTT value, we compare this RTT value and threshold. If the RTT surpassed the threshold, we turn all backup subflows to active.


\subsection{Change MPTCP acknowledgement strategy: Transmission of data-acks on different subflows}
The motivation is to deal with the escalated delay or loss of Data ACKs on one path.
